MOSAIC: Masked Optimisation with Selective Attention for Image Reconstruction

Compressive sensing (CS) reconstructs images from sub-Nyquist measurements by solving a sparsity-regularized inverse problem. Traditional CS solvers use iterative optimizers with hand crafted sparsifiers, while early data-driven methods directly learn an inverse mapping from the low-dimensional measurement space to the original image space. The latter outperforms the former, but is restrictive to a pre-defined measurement domain. More recent, deep unrolling methods combine traditional proximal gradient methods and data-driven approaches to iteratively refine an image approximation. To achieve higher accuracy, it has also been suggested to learn both the sampling matrix, and the choice of measurement vectors adaptively. Contrary to the current trend, in this work we hypothesize that a general inverse mapping from a random set of compressed measurements to the image domain exists for a given measurement basis, and can be learned. Such a model is single-shot, non-restrictive and does not parametrize the sampling process. To this end, we propose MOSAIC, a novel compressive sensing framework to reconstruct images given any random selection of measurements, sampled using a fixed basis. Motivated by the uneven distribution of information across measurements, MOSAIC incorporates an embedding technique to efficiently apply attention mechanisms on an encoded sequence of measurements, while dispensing the need to use unrolled deep networks. A range of experiments validate our proposed architecture as a promising alternative for existing CS reconstruction methods, by achieving the state-of-the-art for metrics of reconstruction accuracy on standard datasets.

==> Images/fig1.tex <==
%!TEX root = ../mosaic.tex
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]
  {Images/overview.pdf}
  \caption{The abstraction of CS: (a) Sampling projects the image $\mathbf{X}$ onto a measurement subspace spanned by the selected rows of $\mathbf{A}$  (b) Given a random choice from the set of possible measurements, the reconstruction model should map from the subspace back onto $\mathbb{R}^n$}.
  \label{fig:1}
\end{figure}
